The Completed SDSS-IV extended Baryon Oscillation Spectroscopic Survey: a multi-tracer analysis in Fourier space for measuring the cosmic structure growth and expansion rate

We perform a joint BAO and RSD analysis using the eBOSS DR16 LRG and ELG samples in the redshift range of $z\in[0.6,1.1]$, and detect a RSD signal from the cross power spectrum at a $\sim4\sigma$ confidence level, i.e., $f\sigma_8=0.317\pm0.080$ at $z_{\rm eff}=0.77$. Based on the chained power spectrum, which is a new development in this work to mitigate the angular systematics, we measurement the BAO distances and growth rate simultaneously at two effective redshifts, namely, $D_{\rm M}/r_{\rm d} \ (z=0.70)=17.96\pm0.51, \ D_{\rm H}/r_{\rm d} \ (z=0.70)=21.22\pm1.20, \ f\sigma_8 \ (z=0.70) =0.43\pm0.05$, and $D_{\rm M}/r_{\rm d} \ (z=0.845)=18.90\pm0.78, \ D_{\rm H}/r_{\rm d} \ (z=0.845)=20.91\pm2.86, \ f\sigma_8 \ (z=0.845) =0.30\pm0.08$. Combined with BAO measurements including those from the eBOSS DR16 QSO and Lyman-$\alpha$ sample, our measurement has raised the significance level of a nonzero $\Omega_{\rm \Lambda}$ to $\sim11\sigma$.

==> implication.tex <==
\section{A cosmological implication}
\label{sec:cosmology}
